Confidence-Ranked Reconstruction of Census Microdata from Published Statistics

A reconstruction attack on a private dataset $D$ takes as input some publicly accessible information about the dataset and produces a list of candidate elements of $D$. We introduce a new class of data reconstruction attacks based on randomized methods for non-convex optimization. We empirically demonstrate that our attacks can not only reconstruct full rows of $D$ from aggregate query statistics $Q(D)\in \mathbb{R}^m$, but can do so in a way that reliably ranks reconstructed rows by their odds of appearing in the private data, providing a signature that could be used for prioritizing reconstructed rows for further actions such as identify theft or hate crime. We also design a sequence of baselines for evaluating reconstruction attacks. Our attacks significantly outperform those that are based only on access to a public distribution or population from which the private dataset $D$ was sampled, demonstrating that they are exploiting information in the aggregate statistics $Q(D)$, and not simply the overall structure of the distribution. In other words, the queries $Q(D)$ are permitting reconstruction of elements of this dataset, not the distribution from which $D$ was drawn. These findings are established both on 2010 U.S. decennial Census data and queries and Census-derived American Community Survey datasets. Taken together, our methods and experiments illustrate the risks in releasing numerically precise aggregate statistics of a large dataset, and provide further motivation for the careful application of provably private techniques such as differential privacy.

==> docs/all_plots.tex <==


\onecolumn

\section{ALL PLOTS}

%%%%%

% \input{figures/census_with_block_init/avg_states.tex}

% \input{figures/census_with_block_init/all_states_1.tex}

% \input{figures/census_with_block_init/all_states_2.tex}

%%%%%

% \input{figures/census_with_block/avg_states.tex}

% \input{figures/census_with_block/all_states_1.tex}

% \input{figures/census_with_block/all_states_2.tex}

% \input{figures/census_with_block/kway_marginals.tex}

\input{figures/census_with_block/vary_num_runs.tex}


%%%%%

% \input{figures/census_ignore_block/avg_states.tex}

% \input{figures/census_ignore_block/all_states_1.tex}

% \input{figures/census_ignore_block/all_states_2.tex}

\input{figures/census_ignore_block/kway_marginals.tex}

%%%%%

% \input{figures/folktables/2-way_marginals.tex}

% \input{figures/folktables/2_3-way_marginals.tex}

\input{figures/folktables/2-way_marginals_subsample.tex}

==> docs/baseline.tex <==

% \begin{algorithm}
% \caption{\matchrate}
% \label{alg:matchrate}
% \begin{algorithmic}
% \Require Original dataset $D$, a reconstruction attack $R=\{x_i\}_{i\in [k]}$.
% % \Ensure $y = x^n$
% \State \textbf{Output:} Reconstruction score of $R$. 
% % \State For any row $x\in R_k$.
% \State Let $m$ be the number of rows in $R$.
% % \State Let $\unique{R} $ be the unique set of rows in $R$.
% \State 

% \For{$k = 1,\ldots, m$}
% \begin{align*}
%     \text{rate}(k) \leftarrow \frac{1}{k}\sum_{i=1}^k \indicator{x_i\in D}
% \end{align*}
% \EndFor
% \State\textbf{Output:} $\matchrate(D, R) \leftarrow \frac{1}{m}\sum_{k=1}^m \text{rate}(k)$
% % \State \textbf{Output:} $\left| D \cap R \right| / \left| R \right|$
% \end{algorithmic}
% \end{algorithm}



\begin{algorithm}
\caption{Sampling baseline}
\label{alg:baseline}
\begin{algorithmic}[1]
\Require A sample dataset $S$.
% \State Sort points in $D$ according to their frequency. 
% \State Let $m$ be the number of unique rows in $S$.
% \State Let $F(x)$ denote the frequency of a row $x$ in $S$.

\State \textbf{Output}  $R$, the set of all unique rows of $S$ sorted by frequency.
\end{algorithmic}
\end{algorithm}




==> docs/reconstruction_metric.tex <==
\begin{algorithm}
\caption{Reconstruction metric}
\label{alg:baseline}
\begin{algorithmic}
\Require Target dataset $D$, a set o$D_2$
% \Ensure $y = x^n$

\State \textbf{Output:}
\end{algorithmic}
\end{algorithm}

==> figures/census_ignore_block/all_states_1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_ignore_block/all_states_1.png}
    \caption{[IGNORES block attribute] We evaluate on a randomly selected tract from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables.}
    \label{fig:census_ib_all_1}
\end{figure}

==> figures/census_ignore_block/all_states_2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_ignore_block/all_states_2.png}
    \caption{[IGNORES block attribute] We evaluate on a randomly selected tract from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables.}
    \label{fig:census_ib_all_2}
\end{figure}

==> figures/census_ignore_block/avg_states.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_ignore_block/avg_states.png}
    \caption{[IGNORES block attribute] We average results across a randomly selected tracts from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables. The figure shows that the \rapattack~ attack guesses more rows of the private data than knowing the county or state distribution but worse than knowing the distribution at the track level.}
    \label{fig:census_ib_avg}
\end{figure}

==> figures/census_ignore_block/kway_marginals.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=\columnwidth]{images/census_ignore_block/kway_marginals.png}
    \caption{[IGNORES block attribute] Comparison on 5 random tracts where we include 2 and 3-way marginal queries.}
    \label{fig:census_ib_kway}
\end{figure}

==> figures/census_with_block/all_states_1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_with_block/all_states_1.png}
    \caption{[INCLUDES block attribute] We evaluate on a randomly selected tract from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables.}
    \label{fig:census_all_1}
\end{figure}

==> figures/census_with_block/all_states_2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_with_block/all_states_2.png}
    \caption{[INCLUDES block attribute] We evaluate on a randomly selected tract from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables.}
    \label{fig:census_all_2}
\end{figure}

==> figures/census_with_block/avg_states.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_with_block/avg_states.png}
    \caption{[INCLUDES block attribute] We average results across a randomly selected tracts from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables. The figure shows that the \rapattack~ attack guesses more rows of the private data than knowing the county or state distribution but worse than knowing the distribution at the track level.}
    \label{fig:census_avg}
\end{figure}

==> figures/census_with_block/kway_marginals.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=\columnwidth]{images/census_with_block/kway_marginals.png}
    \caption{[INCLUDES block attribute] Comparison on 5 random tracts where we include 2 and 3-way marginal queries.}
    \label{fig:census_kway}
\end{figure}

==> figures/census_with_block/vary_num_runs.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/old/census_with_block/vary_num_runs.png}
    \caption{[INCLUDES block attribute] We average results across a randomly selected tracts from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ while varying the number of runs.}
    \label{fig:census_vary_runs}
\end{figure}

==> figures/census_with_block_init/all_states_1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_with_block_init/all_states_1.png}
    \caption{[INCLUDES block attribute] We evaluate on a randomly selected tract from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against the track baseline. We initialize \rapattack rows in the baseline tract. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables.}
    \label{fig:census_all_init_1}
\end{figure}

==> figures/census_with_block_init/all_states_2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_with_block_init/all_states_2.png}
    \caption{[INCLUDES block attribute] We evaluate on a randomly selected tract from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against the track baseline. We initialize \rapattack rows in the baseline tract. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables.}
    \label{fig:census_all_init_2}
\end{figure}

==> figures/census_with_block_init/avg_states.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/census_with_block_init/avg_states.png}
    \caption{[INCLUDES block attribute] We average results across a randomly selected tracts from each state, comparing top $k$ candidate \matchrate~ of \rapattack~ against track, county and state baselines. The $x$-axis corresponds to different value of $k$ and the underlying dataset is a track of the Census tables. We initialize \rapattack rows in the baseline tract.}
    \label{fig:census_avg_init}
\end{figure}

==> figures/folktables/2-way_marginals.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/folktables/2-way_marginals.png}
    \caption{We select state-task combinations from the folktables dataset, comparing top $k$ candidate \matchrate~ of \rapattack~ against the baseline (here, the baseline is derived from the holdout split).}
    \label{fig:folktables_2-way_marginals}
\end{figure}

==> figures/folktables/2-way_marginals_subsample.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/old/folktables/2-way_marginals_subsample.png}
    \caption{We compare top $k$ candidate \matchrate~ of \rapattack~ using random samples (100\%, 50\%, 25\%, and 12.5\%) of $2$-way marginal queries.}
    \label{fig:folktables_2-way_marginals}
\end{figure}

==> figures/folktables/2_3-way_marginals.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=\columnwidth]{images/folktables/2_3-way_marginals.png}
    \includegraphics[width=\columnwidth]{images/folktables/2_3-way_marginals_0.9.png}
    \caption{We select state-task combinations from the folktables dataset, comparing top $k$ candidate \matchrate~ of \rapattack~ against the baseline (here, the baseline is derived from the holdout split).}
    \label{fig:folktables_2_3-way_marginals}
\end{figure}

==> latexmkrc <==


add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


$dvipdf = 'dvipdfmx %O -o %D %S';

==> tables/data.tex <==
\begin{table*}[tbhp]
\caption{Dataset statistics for \textbf{all} $2$-way marginals. $N$ is size of the dataset after splitting the original. 'split\_overlap' is the number of unique rows that the two splits share in common. 'overlap\_\%' is calculated as 'split\_overlap' divided by the number of unique rows in the other split (from which the baseline candidate rows are drawn from). In the aggregate score columns (auc and top), 'bl\_' means baseline, and 'top' means the maximum K for which the top K candidates are all matches.}
% \centering
\begin{tabular}{lrrrrrrrrrrr}
\toprule
       dataset &       N &  num\_attr &  data\_dim &  num\_queries & overlap\_\% &   auc & bl\_auc & auc\_diff &   top &  bl\_top &  top\_diff \\
\midrule
     income\_CA &   97832 &        10 &       839 &       186315 &     7.68\% & 0.719 &  0.629 &   0.0896 &    67 &      68 &        -1 \\
     income\_NY &   51510 &        10 &       839 &       186315 &     8.35\% & 0.700 &  0.606 &   0.0935 &    49 &      49 &         0 \\
     income\_TX &   67962 &        10 &       839 &       186315 &     7.69\% & 0.732 &  0.630 &   0.1013 &    34 &      62 &       -28 \\
     income\_FL &   49462 &        10 &       839 &       186315 &     3.56\% & 0.683 &  0.508 &   0.1757 &    30 &       9 &        21 \\
     income\_PA &   34154 &        10 &       839 &       186315 &    11.18\% & 0.776 &  0.684 &   0.0921 &    23 &      67 &       -44 \\
 employment\_CA &  189408 &        16 &       108 &         5154 &    40.26\% & 0.960 &  0.975 &  -0.0147 &  1525 &    2397 &      -872 \\
 employment\_NY &   98484 &        16 &       108 &         5154 &    36.94\% & 0.909 &  0.904 &   0.0056 &  1192 &    1328 &      -136 \\
 employment\_TX &  134050 &        16 &       108 &         5154 &    39.48\% & 0.944 &  0.950 &  -0.0058 &  1034 &    1993 &      -959 \\
 employment\_FL &  101080 &        16 &       108 &         5154 &    37.06\% & 0.924 &  0.907 &   0.0176 &   976 &    1471 &      -495 \\
 employment\_PA &   64533 &        16 &       108 &         5154 &    38.88\% & 0.924 &  0.905 &   0.0189 &   722 &    1170 &      -448 \\
   coverage\_CA &   69277 &        18 &       107 &         5160 &    27.88\% & 0.875 &  0.845 &   0.0296 &   104 &     655 &      -551 \\
   coverage\_NY &   33776 &        18 &       107 &         5160 &    25.07\% & 0.869 &  0.825 &   0.0442 &   215 &     297 &       -82 \\
   coverage\_TX &   49464 &        18 &       107 &         5160 &    26.35\% & 0.880 &  0.839 &   0.0405 &   369 &     311 &        58 \\
   coverage\_FL &   35648 &        18 &       107 &         5160 &    23.60\% & 0.867 &  0.802 &   0.0645 &   305 &     178 &       127 \\
   coverage\_PA &   22040 &        18 &       107 &         5160 &    26.94\% & 0.897 &  0.846 &   0.0511 &   298 &     198 &       100 \\
     travel\_CA &   86254 &        15 &      1012 &       331930 &     0.62\% & 0.116 &  0.151 &  -0.0348 &     0 &       0 &         0 \\
     travel\_NY &   45600 &        15 &       863 &       219728 &     1.04\% & 0.174 &  0.218 &  -0.0441 &     0 &       0 &         0 \\
     travel\_TX &   60373 &        15 &       971 &       302479 &     0.72\% & 0.161 &  0.231 &  -0.0694 &     0 &       1 &        -1 \\
     travel\_FL &   44036 &        15 &       911 &       256964 &     0.51\% & 0.113 &  0.107 &   0.0062 &     0 &       0 &         0 \\
     travel\_PA &   29950 &        15 &       821 &       189649 &     1.03\% & 0.300 &  0.247 &   0.0529 &     3 &       0 &         3 \\
   mobility\_CA &   40164 &        21 &       141 &         9137 &    15.97\% & 0.821 &  0.743 &   0.0780 &    53 &      60 &        -7 \\
   mobility\_NY &   20232 &        21 &       141 &         9137 &    13.63\% & 0.797 &  0.700 &   0.0975 &   105 &      42 &        63 \\
   mobility\_TX &   26656 &        21 &       141 &         9137 &    16.22\% & 0.822 &  0.724 &   0.0980 &    32 &      17 &        15 \\
   mobility\_FL &   17246 &        21 &       141 &         9137 &    12.22\% & 0.768 &  0.599 &   0.1685 &     8 &      15 &        -7 \\
   mobility\_PA &   11959 &        21 &       141 &         9137 &    17.22\% & 0.774 &  0.696 &   0.0781 &     3 &      21 &       -18 \\
\bottomrule
\end{tabular}

\addtabletext{Additional notes: split\_overlap and overlap\_\% help give some sense of how much the two splits share in common and should positively correlate with the performance of data splitting baseline (TBD if this is true).}
\end{table*}
